Interactive Task Planning with Language Models

An interactive robot framework accomplishes long-horizon task planning and can easily generalize to new goals and distinct tasks, even during execution. However, most traditional methods require predefined module design, making it hard to generalize to different goals. Recent large language model based approaches can allow for more open-ended planning but often require heavy prompt engineering or domain specific pretrained models. To tackle this, we propose a simple framework that achieves interactive task planning with language models by incorporating both high-level planning and low-level skill execution through function calling, leveraging pretrained vision models to ground the scene in language. We verify the robustness of our system on the real world task of making milk tea drinks. Our system is able to generate novel high-level instructions for unseen objectives and successfully accomplishes user tasks. Furthermore, when the user sends a new request, our system is able to replan accordingly with precision based on the new request, task guidelines and previously executed steps. Our approach is easy to adapt to different tasks by simply substituting the task guidelines, without the need for additional complex prompt engineering. Please check more details on our https://wuphilipp.github.io/itp_site and https://youtu.be/TrKLuyv26_g.

==> figures/progpromptsim/figure.tex <==
\begin{figure}[pb]
\centering%
\includegraphics[width=1.0\linewidth]{figures/progpromptsim/progprompt.png}
% \vspace*{-4ex}
\caption{ProgPrompt JSON File. } 
\label{fig:progpromptsim}
\end{figure}
